A Comprehensive Evaluation on Multi-channel Biometric Face Presentation Attack Detection

The vulnerability against presentation attacks is a crucial problem undermining the wide-deployment of face recognition systems. Though presentation attack detection (PAD) systems try to address this problem, the lack of generalization and robustness continues to be a major concern. Several works have shown that using multi-channel PAD systems could alleviate this vulnerability and result in more robust systems. However, there is a wide selection of channels available for a PAD system such as RGB, Near Infrared, Shortwave Infrared, Depth, and Thermal sensors. Having a lot of sensors increases the cost of the system, and therefore an understanding of the performance of different sensors against a wide variety of attacks is necessary while selecting the modalities. In this work, we perform a comprehensive study to understand the effectiveness of various imaging modalities for PAD. The studies are performed on a multi-channel PAD dataset, collected with 14 different sensing modalities considering a wide range of 2D, 3D, and partial attacks. We used the multi-channel convolutional network-based architecture, which uses pixel-wise binary supervision. The model has been evaluated with different combinations of channels, and different image qualities on a variety of challenging known and unknown attack protocols. The results reveal interesting trends and can act as pointers for sensor selection for safety-critical presentation attack detection systems. The source codes and protocols to reproduce the results are made available publicly making it possible to extend this work to other architectures.

==> Makefile <==
# Builds the LaTeX project as a PDF document

TEXFILE=main.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex 
	@if [ ! -e $(@:%.pdf=%.aux) ]; then \
	 pdflatex $(@:%.pdf=%.tex); \
	 fi
	@if [ -e ref.bib ]; then \
	 bibtex $(@:%.pdf=%); \
	 pdflatex $(@:%.pdf=%.tex); \
	fi
	pdflatex $(@:%.pdf=%.tex)
	pdflatex $(@:%.pdf=%.tex)
	pdflatex $(@:%.pdf=%.tex)

all: $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.dvi *.ps *.out *.brf *.spl
	@rm -vf *.nav *.snm
	@rm -vf main.pdf

